Adaptivity in Adaptive Submodularity

Adaptive sequential decision making is one of the central challenges in machine learning and artificial intelligence. In such problems, the goal is to design an interactive policy that plans for an action to take, from a finite set of $n$ actions, given some partial observations. It has been shown that in many applications such as active learning, robotics, sequential experimental design, and active detection, the utility function satisfies adaptive submodularity, a notion that generalizes the notion of diminishing returns to policies. In this paper, we revisit the power of adaptivity in maximizing an adaptive monotone submodular function. We propose an efficient semi adaptive policy that with $O(\log n \times\log k)$ adaptive rounds of observations can achieve an almost tight $1-1/e-\epsilon$ approximation guarantee with respect to an optimal policy that carries out $k$ actions in a fully sequential manner. To complement our results, we also show that it is impossible to achieve a constant factor approximation with $o(\log n)$ adaptive rounds. We also extend our result to the case of adaptive stochastic minimum cost coverage where the goal is to reach a desired utility $Q$ with the cheapest policy. We first prove the conjecture of the celebrated work of Golovin and Krause by showing that the greedy policy achieves the asymptotically tight logarithmic approximation guarantee without resorting to stronger notions of adaptivity. We then propose a semi adaptive policy that provides the same guarantee in polylogarithmic adaptive rounds through a similar information-parallelism scheme. Our results shrink the adaptivity gap in adaptive submodular maximization by an exponential factor.

==> lemma.tex <==
In this section, we show how the expected utility obtained by the greedy algorithm is related to the expected utility obtained by the optimum policy. Let us define $\pi^{\tau}$ to be the policy that runs the greedy policy $\pigreedy$ and stops when the expected marginal gain of all of the remaining elements is less than or equal to $\tau$. We define $\tau_i$ to be a threshold such that the expected number of elements selected by $\pi^{\tau_i}$ is $i$, in other words $\sum_{\phi}p(\phi)|S(\pi^{\tau_i},\phi)|=i$.\footnote{Use an arbitrary tie breaking rule to make it exactly equal. For example, if by accepting elements whose expected marginal benefit is strictly larger than $\tau$ the greedy policy selects $\alpha<i$ elements in expectation, and by accepting elements with expected marginal  benefit larger than or equal to $\tau$ the greedy policy selects $\beta>i$ elements in expectation, then we let the policy $\pi^{\tau_i}$ accepts $\tau$ with probability $\frac{i - \alpha}{\beta - \alpha}$. Hence, the expected number of items accepted by $\pi^{\tau_i}$ is $\alpha + \frac{i - \alpha}{\beta - \alpha} (\beta-\alpha) = i$.} In this section, as well as the rest of the paper, we assume that our function of interest $f$, is an adaptive monotone and adaptive submodular function with respect to the distribution $p(\phi)$. 
%
For two policies $\pi$ and $\pi'$ we define $\pi@\pi'$  to be a policy that first runs $\pi$ and then runs $\pi'$ from a fresh start (i.e., ignoring the information gathered by $\pi$). This definition implies $S(\pi@\pi',\phi)=S(\pi,\phi)\cup S(\pi',\phi)$.

Whenever we use expectation notation $\E[\chi]$ for a random variable $\chi$, 
the expectation is over all randomness of $\chi$, unless specified otherwise. 
Moreover, note that we always use capital letters for random variables, and small 
letters for realizations. For example $\Psi$ refers to a random variable, and 
$\psi$ refers to a realization of $\Psi$, and hence $\psi$ is a deterministic 
quantity.
%\textcolor{red}{(what is the difference between $\phi$ and $\psi$). I think we used $\phi$ for realizations and $\psi$ for partial realizations. But then in the text they are not consistently used. There is a difference between partial realizations and realizations}.

The following is the key lemma of this section.
\begin{lemma}\label{lm:1-1/e^l}
	For any policy $\pi^*$ and any positive integer $\ell$ we have 
	\begin{align*}
	f_{avg}(\pi^{\tau_{\ell}}) > \big(1-e^{-\frac{\ell}{\ex{K}+1}}\big) f_{avg}(\pi^*),
	\end{align*}
	where $K$ is a random variable that indicates the 
	number of items picked by $\pi^*$, i.e. $K=|S(\pi^*, \Phi)|$. 
\end{lemma}

%\begin{comment}
Before proving Lemma~\ref{lm:1-1/e^l}, we provide some primitives that we use in the proof of this lemma as well as Lemmas~\ref{lm:par:1-1/e^l} and~\ref{lm:batch:1-1/e^l}.


For a randomized policy $\pi$, we use $\Theta_{\pi}$ to indicate the random seed of the policy $\pi$. We use $\theta_{\pi}$ to indicate a realization of $\Theta_{\pi}$ and use $p(\theta_{\pi})$ to indicate the probability that $\theta_{\pi}$ is realized. We drop $\pi$ from the notation when it is clear from the context.
%

For a deterministic policy $\pi$, a randomized policy $\pi^*$, an element $e$, and two subrealization $\psi$ and $\psi'\sim \psi$, we define event $<\psi,\psi',e,\pi,\pi^*>$ to be the event that
\begin{itemize}
	\item the set of elements selected by policy $\pi@\pi^*$, at some point during its run, is the same as the elements of $\psi'$ and then $\pi@\pi^*$ immediately selects $e$,
	\item and, $\pi$ selects the elements of $\psi$ at its termination. 
\end{itemize}


%
Note that for a fixed seed $\theta_{\pi^*}$, conditioned on $\Phi\sim \psi'$, we can simulate $\pi@\pi^*$ and deterministically indicate whether event $<\psi,\psi',e,\pi,\pi^*>$ happens or not.\footnote{Note that if policy $\pi@\pi^*$ attempts to query an element that does not exist in $\psi'$, we know that the event $<\psi,\psi',e,\pi,\pi^*>$ does not happen and do not need to simulate the policy any further.} We define $\1_{\psi',\psi,e,\pi,\pi^*,\theta_{\pi^*}}$ to be a \emph{deterministic} binary variable that is $1$ if and only if, conditioned on $\Theta_{\pi^*}=\theta_{\pi^*}$ and $\Phi\sim \psi'$, event $<\psi,\psi',e,\pi,\pi^*>$ happens. We drop the notations of policies and use $\1_{\psi',\psi,e,\theta}$, when they are clear from the context.


%In the following lemma use the notations $\1$ and $\theta$ for policy $\pi^{\tau_i}@\pi^*$, for a certain $i$, hence for the simplicity of notation we drop the notation of the policy from the subscripts and use $\theta$ and $\1_{\psi,e,\theta}$. In other words, we define $\theta:=\theta_{\pi^{\tau_i}@\pi^*}$ and $\1_{\psi,e,\theta}:=\1_{\psi,e,\pi^{\tau_i}@\pi^*,\theta_{\pi^{\tau_i}@\pi^*}}$.

\begin{comment}
We define $\1_{\pi, e,\psi}$ to be a binary random variable that is $1$ if the event $<\pi, e,\psi>$ happens and is $0$ if the event $<\pi, e,\psi>$ does not happen.  \textbf{Note that}, conditioned on $\Phi\sim \psi$, the value of $\1_{\pi,e,\psi}$ is independent of the randomness of $\Phi$ and solely depends on the randomness of policy $\p$. For example, if $\pi$ is a deterministic policy, conditioned on $\Phi\sim \psi$, the value of $\1_{\pi,e,\psi}$ is deterministic. 

We define the random variable $\gamma(e|\psi)$ to be $f(\psi'\cup \Phi(e))-f(\psi')$ conditioned on $\Phi\sim \psi'$ and $\1_{e,\psi}=1$. Recall that, $\Delta(e|\psi)= \ex{f(\psi\cup \Phi(e))-f(\psi)\Big|\Phi\sim \psi}$. Hence, we have
\begin{align}
\ex{\gamma(e|\psi)}&=
\ex{f(\psi'\cup \Phi(e))-f(\psi')|\Phi\sim \psi' \text{ and } \1_{e,\psi}=1}\nonumber\\
&=\ex{f(\psi'\cup \Phi(e))-f(\psi')|\Phi\sim \psi'}\nonumber\\
&=\Delta(e|\psi).
\end{align}
\end{comment}


\begin{proofof}{Lemma~\ref{lm:1-1/e^l}}
	First we provide an upper bound on $f_{avg}(\pi^*)$. Pick an arbitrary number $i\in \{0,\dots,\ell\}$. Note that by adaptive monotonicity, we have $f_{avg}(\pi^*) \leq f_{avg}(\pi^{\tau_i}@\pi^*)$. Next we show that $f_{avg}(\pi^{\tau_i}@\pi^*) \leq f_{avg}(\pi^{\tau_i})+\ex{K}\Delta^{\tau_i}(\pi)$, where $\Delta^{\tau_i}(\pi)=f_{avg}(\pi^{\tau_{i}})-f_{avg}(\pi^{\tau_{i-1}})$. This implies that 
	\begin{align}\label{eq:main}
	f_{avg}(\pi^*) \leq f_{avg}(\pi^{\tau_i}@\pi^*) \leq f_{avg}(\pi^{\tau_i})+\ex{K}\Delta^{\tau_i}(\pi).
	\end{align}
	
	Let $\Psi_i$ be a random variable that indicates the partial realization observed by running policy $\pi^{\tau_i}$. We use $\psi_i$ to indicate a realization of the random variable $\Psi_i$. Note that, 
	by definition of $\pi^{\tau_i}$ we have ${\tau_i}\geq \max_{e\in E\setminus 
		\dom(\psi_i)} \Delta(e|\psi_i)$. Moreover, by adaptive submodularity for any 
	consistent partial realization $\psi'\sim \psi_i$ and for all $e\in 
	E\setminus\dom(\psi')$ we have $\Delta(e|\psi_i)\geq \Delta(e|\psi')$. 
	Therefore, we have
	
	\begin{equation}\label{eq:greedE}
	{\tau_i} \geq \Delta(e|\psi'), \quad\quad{\forall{\psi'\sim 
			\psi_i}\text{ and }\forall{e\in 
			E\setminus\dom(\psi')} }.
	\end{equation} 
	

	We have
	\begin{align*}
		&f_{avg}(\pi^{\tau_i}@\pi^*) - f_{avg}(\pi^{\tau_i}) \\
		&= \sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')}\sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\ex{f(\psi'\cup \Phi(e))-f(\psi')|\Phi\sim \psi' \text{ and } \Theta_{\pi^*}=\theta} &\text{Definition}\\ 
		&= \sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')}\sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\ex{f(\psi'\cup \Phi(e))-f(\psi')|\Phi\sim \psi'} &\hspace{-1cm}\text{Independency\footnotemark}\\ 
		&=  \sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')} \sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\Delta(e|\psi') &\text{Definition}\\
		&\leq \sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')} \sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\tau_i &\text{Inequality \ref{eq:greedE}}\\
		&\leq \sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')} \sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\Delta^{\tau_i}(\pi) & \Delta^{\tau_i}(\pi) \geq \tau_i  \\
		&= \Big(\sum_{\psi_i\in \Psi_i}\sum_{\psi' \sim \psi_i}\sum_{e\notin \dom(\psi')} \sum_{\theta\in \Theta_{\pi^*}} p(\psi')p(\theta)\1_{\psi_i,\psi',e,\theta}\Big)\Delta^{\tau_i}(\pi) \\
		& = \ex{K}\Delta^{\tau_i}(\pi).
	\end{align*} \footnotetext{Note that $\psi'$ is fixed, hence $f(\psi'\cup\Phi(e))-f(\psi')$ is independent of $\Theta$.}
	This proves inequality \eqref{eq:main} as promised.	
	
	Let us define $\Delta_i^*=f_{avg}(\pi^*)-f_{avg}(\pi^{\tau_i})$. Inequality 
	\ref{eq:main} implies that $\Delta_{i}^*\leq 
	\ex{K}(\Delta_{i-1}^*-\Delta_{i}^*)$. By a simple rearrangement we have 
	$\Delta_{i}^*\leq\big(1-\frac 1 {\ex{K}+1}\big)\Delta_{i-1}^*$. By iteratively 
	applying this inequality we have $$\Delta_{\ell}^*\leq\big(1-\frac 1 
	{\ex{K}+1}\big)^{\ell}\Delta_{0}^*\leq e^{-\frac{\ell}{\ex{K}+1}} \Delta_{0}^*.$$ 
	By applying the definition of $\Delta_{i}^*$ and some rearrangements we have 
	$f_{avg}(\pi^{\tau_{\ell}}) > \big(1-e^{-\frac{\ell}{\ex{K}+1}}\big) 
	f_{avg}(\pi^*)$ as desired.
\end{proofof} 
